CAOS: Concurrent-Access Obfuscated Store

This paper proposes Concurrent-Access Obfuscated Store (CAOS), a construction for remote data storage that provides access-pattern obfuscation in a honest-but-curious adversarial model, while allowing for low bandwidth overhead and client storage. Compared to the state of the art, the main advantage of CAOS is that it supports concurrent access without a proxy, for multiple read-only clients and a single read-write client. Concurrent access is achieved by letting clients maintain independent maps that describe how the data is stored. These maps might diverge from client to client, but it is guaranteed that no client will ever lose track of current data. We achieve efficiency and concurrency at the expense of perfect obfuscation: in CAOS the extent to which access patterns are hidden is determined by the resources allocated to its built-in obfuscation mechanism. To assess this trade-off we provide both a security and a performance analysis of our protocol instance. We additionally provide a proof-of-concept implementation.

==> csw-main.tex <==
\begin{algorithm2e}
%\DontPrintSemicolon
\SetKwProg{function}{function}{}{}
\SetKwProg{rnd}{in random order}{}{}

\KwIn{block id, operation, data (for write operation), store, client map, store key}
\KwOut{data (for read operation), store, client map}

\SetKwProg{fn}{function}{}{}

\BlankLine
\function{$\ACCESSRW$ (bid, op, data, S,  $map_c$, k)}{	
	\BlankLine
	$req\_p \gets SelectPosition (bid, map_c)$\; \label{a1l1}
	$cpy\_p \gets SelectPosition (null, map_c)$\; \label{a1l2}
	
	\BlankLine
	$(req\_blk,cpy\_blk) \gets$ READ($req\_p,cpy\_p,S,k$)\; \label{a1l3}
	
	\BlankLine
	$(req\_blk,map_c) \gets Sync(req\_blk, req\_p, map_c)$\; \label{a1l4}
	$(cpy\_blk,map_c) \gets Sync(cpy\_blk, cpy\_p, map_c)$\; \label{a1l5}
	
	\BlankLine
	\If {$(op = READ)$}{\label{a1lif}
		\If {$(req\_blk.bid = bid)$}{
			$out \gets req\_blk.data$\;
		}\label{a1lif1}
	}
	\If {$(op = WRITE)$}{\label{a1lel}
		$(req\_blk,out) \gets PrepareWrite (bid, req\_blk, data)$\;
	}\label{a1life}
	
	\BlankLine
	$(cpy\_blk, map_c) \gets DuplicateBlock(req\_blk, cpy\_blk, cpy\_p, map_c)$\;\label{a1dup}
	
	\BlankLine
	$S\gets$WRITE($S,k,req\_blk, cpy\_blk, req\_p, cpy\_p$)\;\label{a1wrt}
	
	\BlankLine
	\Return $(out, S, map_c)$\;\label{a1ret}
	
}
\caption{Main ObRAM access function.}
\label{algo:csw-main}
\end{algorithm2e}


==> csw-read.tex <==
\begin{algorithm2e}
\small
%\DontPrintSemicolon
\SetKwProg{function}{function}{}{}

\KwIn{block id, client $map_c$}
\KwOut{position}

\SetKwProg{fn}{function}{}{}

\BlankLine
\function{SelectPosition (bid, $map_c$)}{

	\If {$bid$}{
		$p \xleftarrow{R} map_c[bid].psns$\;
	}\Else {
		$p \xleftarrow{R} position$\;
	}
	\Return p\;
}
\caption{Read a block from the store.}
\label{algo:csw-read}
\end{algorithm2e}


==> related.tex <==
\section{Related Work and Usage Examples}
\label{app:related}

To our knowledge, there is no existing work that uses an obfuscation client to hide access patterns. However several works have been influential in the development of \schemeacr{}.

\smallskip\noindent\textit{Oblivious RAM (ORAM).} Since the initial proposal of Goldreich and Ostrovsky \cite{goldreich1987towards, goldreich1996software}, work on ORAM has been mainly focused on addressing access-pattern privacy related issues in cloud storage \cite{stefanov2013path,stefanov2013oblivistore, dautrich2014burst, ren2015constants,williams2012privatefs,sahin2016taostore}. However, in spite significant progress, ORAMs still have considerable bandwidth requirements which usually makes them impractical for real life applications \cite{senny2014blog}. The \textit{map} data structure used to track where blocks are stored has also restricted applications of ORAM to scenarios that mostly involve a single-client accessing a server, although asynchronous schemes have been proposed \cite{stefanov2013oblivistore}. TaoStore \cite{sahin2016taostore} was the first to to introduce a formal study about asynchronicity in ORAM systems, and a scheme called Tree-based Asynchronous Oblivious Store (TaoStore) which was proven secure under this asynchronous access model.

\schemeacr{} uses concepts from ORAMs, such as the generic block storage, and the client stored maps which track where blocks are stored on the remote server. However, \schemeacr{} uses a different security model than ORAM, achieves better bandwidth efficiency (i.e. $O(1)$ for the RW/RO class of clients), and uses maps together with a synchronisation protocol which enables concurrent client access to the store.

\begin{comment}
%reducing bandwidth
PathORAM \cite{stefanov2013path} was the first ORAM algorithm to propose a tree-based structure for the server store. This construction has a bandwidth which is logarithmically proportional to the size of the data stored and reduced impact on the client's storage. Optimizations to PathORAM \cite{ren2014ring, ren2015constants, devadas2016onion} allow to further decrease the bandwidth requirements with specially chosen parameters. In spite of these improvements, in real life scenarios even the best ORAMs can prove to be impractical \cite{senny2014blog}, mainly because of the high bandwidth requirements and/or client storage constraints. As such, finding more bandwidth efficient constructions (with acceptable client storage requirements) is still one of the main open problems.

%concurrent access
Another limitation of the most recent ORAM constructions is their reliance on a \textit{map} -- a client maintained local data structure which is used to track where blocks are stored in the server store. Within ORAM, every access operation modifies the map in an unpredictable way (i.e., blocks are randomly reassigned to different paths). This makes concurrent client access with ORAMs very difficult. Scenarios where multiple clients are considered, require reliable means to obtain up-to-date versions of the map before being able to access the remote data store. The standard approach to mitigate this problem is to enable access to the remote storage through a proxy or gateway that is positioned in a trusted zone. In this approach the proxy will be the only "client" that stores the map \cite{williams2012privatefs} and all accesses to the store will be mediated by it. However, this solution has raised security considerations about leakage incurred especially when multiple clients access the store concurrently \cite{sahin2016taostore}. As such, direct, proxy-less, connections are preferred.



\smallskip\noindent\textit{Searchable Encryption (SE).} Searchable encryption is a related field with the main focus of providing access-pattern privacy when accessing a search index stored in the cloud \cite{bosch_survey_2014}. SE schemes aim to off-load as much client computation as possible to the remote server. \schemeacr{} has adopted this principle and offloads the heavy computation that would otherwise be performed by RW/RO clients to OCs.


SE schemes usually use deterministic trapdoors perform searches on fixed indexes which are usually difficult to regenerate \cite{curtmola_searchable_2006,david_cash_highly-scalable_2013}. Once a search has been completed SE schemes require may require an additional PIR protocol to access data. This is why ORAM is sometimes proposed as a solution for enabling secure cloud search \cite{senny2014blogse}. As a general purpose data storage protocol, ORAM can store search indexes and facilitate access to them (although not as efficiently as a SE scheme would) and also provide secure information retrieval.


\schemeacr{} is also general purpose storage protocol which can encode a search index as store blocks. Using \schemeacr{} as a storage for an encrypted search index can provide several advantages over both ORAM and standard SE schemes such as: similar bandwidth efficiency to SE schemes, non-deterministic trapdoors assuming that \schemeacr{} position identifiers are used as trapdoors, cheap and secure extensions to the search index, and the ability to be used as a PIR protocol.

\end{comment}

\begin{comment}

 However, the bandwidth requirements in ORAM are much higher, which makes ORAM not suitable for SE in most scenarios.


\medskip \noindent\textbf{PathORAM \cite{stefanov2013path} and PathORAM variations.} PathORAM has been proposed to address limitations in client storage. It builds on a scheme previously proposed by Shi et al. \cite{stefanov2011towards} which has logarithmic bandwidth requirements but requires O(1) client storage. The main properties of PathORAM are that the server stores data in a tree-based structure. PathORAM requires client storage for the stash and has measurable bandwidth requirements of $2\cdot Z\cdot logN$ where $Z$ is the number of blocks stored in a bucket
% (i.e. tree node/leaf) 
and N is the size of the store (in nodes).

%BurstORAM\cite{dautrich2014burst} builds on the Oblivistore \cite{stefanov2013oblivistore} algorithm. In BurstORAM and Oblivistore the ORAM blocks are partitioned into $O(\sqrt N)$ partitions with $O(\sqrt N)$ blocks each, which act as smaller ORAMs of $O(log N)$ levels (partitioning enables parallel access). Both Oblivistore and BurstORAM delay eviction operations and shuffling by caching data on the client to save bandwidth. BurstORAM additionally uses a XOR technique to combine $O(logN)$ blocks into a single block during the request block operation.

RingORAM \cite{ren2015constants} is an improvement of PathORAM which proposes a method to reduce the overall bandwidth requirements with values between 2.3$\times$ to 4$\times$ by combining a couple of techniques: only one block is read from each bucket in the path; and the evict operation has been optimised to select paths in a reverse lexicographic order. Additionally the evict operation is no longer triggered with every access operation.

OnionORAM\cite{devadas2016onion} is an ORAM construction that achieves constant bandwidth blow-up. Onion ORAM improves the eviction procedure used in other ORAMs \cite{stefanov2013path, ren2015constants, stefanov2013oblivistore, dautrich2014burst} by moving blocks from a source bucket to its children in a specific way which allows assumptions to be made about the state of the buckets on the eviction path -- {after an eviction the buckets on the eviction path are guaranteed to be empty}. The new eviction method named bucket-triplet eviction can be combined with additive homomorphic encryption to achieve the constant bandwidth blow-up.

\noindent\textbf{PrivateFS \cite{williams2012privatefs}.} PrivateFS is an oblivious file system which uses a parallel access ORAM construction PD-ORAM. PD-ORAM allows multiple clients to share an {ORAM Instance}, a trusted third-party which provides an interface to clients. The {ORAM Instance} is responsible for managing the ORAM access keys and acts as an {ORAM access} operation scheduler for the clients that want to use the ORAM store.

\noindent\textbf{TaoStore \cite{sahin2016taostore}.} TaoStore  proposes the first formal study for asynchronicity in ORAM systems. The paper introduces a new security model and new security definitions for studying asynchronous accesses from trusted groups to ORAM stores. The authors show that several ORAM schemes \cite{stefanov2013oblivistore, bindschaedler2015practicing} are insecure under this new model - the asynchronous scheduling of network communications.
The paper also describes a new ORAM system called Tree-based Asynchronous Oblivious Store (TaoStore) that is proven secure under the proposed model.

\noindent\textbf{Anonymous RAM \cite{williams2012privatefs}.} Anonymous RAM (AnonRAM) is a multi-storage primitive for ORAM that simultaneously protects privacy of content, access patterns and user's identity. The system guarantees integrity in multi-user ORAM stores by preventing malicious users from corrupting data of other users.
\end{comment}

